SAM-Enhanced Segmentation on Road Datasets: Balancing Critical Classes in Autonomous Driving

Dense semantic segmentation is essential for autonomous driving, yet many multi-modal datasets lack pixel-level annotations. The Zenseact Open Dataset (ZOD) provides rich multi-sensor data but only bounding-box labels, limiting its use for segmentation research. Our primary contribution is a Segment Anything Model (SAM)-based annotation pipeline that produces dense, pixel-level annotations for ZOD by converting bounding boxes into semantic masks. In this pilot study, we process over 100,000 frames and manually curate a 2,300-frame subset (36% acceptance rate) to establish a reliable baseline. Using these annotations, we evaluate transformer-based CLFT and CNN-based DeepLabV3+ architectures across diverse weather conditions, achieving up to 48.1% mIoU with CLFT-Hybrid. To address extreme class imbalance, where pedestrians, cyclists, and signs constitute less than 1% of pixels, we explore specialized models targeting rare classes. We further validate the pipeline on the Iseauto autonomous-vehicle platform, achieving 77.5% mIoU, and show that SAM-derived representations transfer effectively across sensor configurations via bidirectional transfer learning. All code and annotations are released to support reproducible research.

==> tables/training_config.tex <==
\begin{table*}[htbp]
\centering
\caption{Training Configuration Parameters for Main Architectures}
\label{tab:training_config}
\begin{tabular}{@{}l c c c c c c c @{}}
\toprule
Architecture & Backbone & Input Size & Batch Size & Learning Rate & Epochs & Optimizer & LR Scheduler \\
\midrule
CLFT-Base & ViT-Base (patch16) & 384×384 & 8 & $8\times10^{-5}$ & 200 & Adam & Step ($\gamma=0.1$, step=50) \\
CLFT-Large & ViT-Large (patch16) & 384×384 & 8 & $8\times10^{-5}$ & 200 & Adam & Step ($\gamma=0.1$, step=50) \\
CLFT-Hybrid & ResNet-101 + ViT-Base & 384×384 & 8 & $8\times10^{-5}$ & 200 & Adam & Step ($\gamma=0.1$, step=50) \\
DeepLabV3+ & ResNet-101 & 384×384 & 8 & $8\times10^{-5}$ & 100 & Adam & Step ($\gamma=0.5$, step=15) \\
\midrule
\multicolumn{8}{l}{\textbf{Data Augmentation:} Random crop (30\% prob), horizontal flip (50\% prob), rotation (±20°), color jitter} \\
\multicolumn{8}{l}{\textbf{Loss Function:} Cross-entropy with class weights (background: 0.1, vehicle: 10.0, sign: 15.0, human: 20.0)} \\
\multicolumn{8}{l}{\textbf{Dataset Split:} 60\% train, 20\% validation, 20\% test (2,300 ZOD frames total)} \\
\bottomrule
\end{tabular}
\end{table*}
